Prompt Pre-Training with Twenty-Thousand Classes for Open-Vocabulary Visual Recognition

This work proposes POMP, a prompt pre-training method for vision-language models. Being memory and computation efficient, POMP enables the learned prompt to condense semantic information for a rich set of visual concepts with over twenty-thousand classes. Once pre-trained, the prompt with a strong transferable ability can be directly plugged into a variety of visual recognition tasks including image classification, semantic segmentation, and object detection, to boost recognition performances in a zero-shot manner. Empirical evaluation shows that POMP achieves state-of-the-art performances on 21 datasets, e.g., 67.0% average accuracy on 10 classification datasets (+3.1% compared to CoOp) and 84.4 hIoU on open-vocabulary Pascal VOC segmentation (+6.9 compared to ZSSeg). Our code is available at https://github.com/amazon-science/prompt-pretraining.

==> tables/cocoop.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[]
\centering
\begin{tabular}{@{}lcccc@{}}
\toprule
Method      & Accuracy (\%) & Tunable params (M) & GPU memory (G) & Training time (h) \\ \midrule
CoCoOp        & 70.14         & 0.07              & 28.3           & 27.5               \\
% CoCoOp (base2new)        & 0.07         & ?              & 28.3           & ?               \\ 
\midrule
% POMP (K=32)  & 63.49         & 0.012              & 3.6            & 2.7               \\
% POMP (K=128) & 64.39         & 0.012              & 5.3            & 2.7               \\
POMP (K=128) & 69.54         & 0.07              & 5.5            & 7.9               \\
% POMP (base2new) (K=128) & ?         & 0.07              & 2.7            & ?               \\
% para: 4x768+768x(768//16)x2 / 1024 / 1024=0.07
\bottomrule
\end{tabular}
\caption{few-shot ImageNet}
\end{table*}

==> tables/cross-dataset-od.tex <==
\begin{table*}[th]
\small
\centering
\begin{tabular}{l|cc|cccccc|cccccc}
\toprule
\multirow{2}{*}{Method}&\multicolumn{2}{c|}{Pascal VOC}&\multicolumn{6}{c|}{COCO}&\multicolumn{6}{c}{Objects365}\\
&AP$_{50}$&AP$_{75}$&AP&AP$_{50}$&AP$_{75}$&AP$_s$&AP$_m$&AP$_l$&AP&AP$_{50}$&AP$_{75}$&AP$_s$&AP$_m$&AP$_l$\\
\midrule
Supervised&78.5&49.0&46.5&67.6&50.9&27.1&67.6&77.7&25.6&38.6&28.0&16.0&28.1&36.7\\
\midrule
ViLD*~\cite{gu2021zero} & 73.9 & 57.9  & 34.1 & 52.3 & 36.5 & 21.6 & 38.9 & 46.1 & 11.5 & 17.8 & 12.3 & 4.2 & 11.1 & 17.8\\
DetPro~\cite{Du2022LearningTP}  & 74.6  & 57.9  & 34.9  & 53.8  & 37.4  & 22.5  & 39.6  & 46.3  & 12.1  & 18.8  & 12.9  & 4.5  & 11.5  & 18.6 \\
\midrule
Detic~\cite{Zhou2022DetectingTC}  &         &       &    38.8     &    56.0     &      41.9   &    25.6     &      42.2   &    50.0   & 15.6  & 22.1  & 16.8  & 6.1  & 15.6  & 23.8  \\
POMP (Ours)          &         &       &    \textbf{40.3}     &      \textbf{57.9}   &    \textbf{43.6}     &      \textbf{28.3}   &    \textbf{43.9}     &  \textbf{50.6}     & \textbf{16.1}    & \textbf{22.9}    & \textbf{17.3}    & \textbf{6.2}    & \textbf{16.3}    & \textbf{24.7}                     \\
\bottomrule
\end{tabular}
\caption{We evaluate the LVIS-trained model on Pascal VOC test set, COCO validation set and Object365 validation set.}
\label{tab:generalization}
\end{table*}

==> tables/finetune.tex <==
\begin{table*}[htbp]
    \centering
    % \footnotesize
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{ccllllllllllll}
        Method & \# Shot & 
        \rotatebox{90}{ImageNet} & 
        \rotatebox{90}{CIFAR-10} & 
        \rotatebox{90}{CIFAR-100} & 
        %  \rotatebox{90}{STL-10} &
         \rotatebox{90}{Food-101} &
         \rotatebox{90}{Stanford Cars} &
         \rotatebox{90}{FGVC Aircraft} &
         \rotatebox{90}{Oxford Pets} &
         \rotatebox{90}{Caltech-101} &
         \rotatebox{90}{Oxford Flowers} &
         \rotatebox{90}{EuroSAT} &
         \rotatebox{90}{DTD} &
         \rotatebox{90}{Average} \\
         \toprule
      Zero-Shot   & 0  & 59.8 & 71.6 & 40.6 & 80.6 & 54.3 & 17.0 & 85.5 & 84.5 & 65.5 & 41.8 & 41.2 \\
      \midrule
                  & 1  & 22.1 & 44.3 & 18.2 & 31.4 & 24.3 & 13.0 & 30.2 & 56.7 & 56.1 & 46.8 & 29.8 & \\
                  & 2  & 31.9 & 53.5 & 26.6 & 45.1 & 36.8 & 17.9 & 40.5 & 68.7 & 74.9 & 55.5 & 41.4 & \\
Linear            & 4  & 41.4 & 62.2 & 35.6 & 56.8 & 49.5 & 23.9 & 56.4 & 79.0 & 86.3 & 65.7 & 51.9 & 55.3 \\
Probe             & 8  & 49.4 & 70.1 & 43.6 & 67.1 & 61.2 & 29.4 & 67.5 & 84.3 & 91.5 & 75.1 & 59.0 & \\
                  & 16 & 55.9 & 73.8 & 50.5 & 73.7 & 70.0 & 36.0 & 75.1 & 87.3 & 95.6 & 80.7 & 64.3 & \\
          \midrule
                  & 1  & 53.4 & 71.8 & 41.3 & 77.5 & 54.0 & 17.7 & 86.5 & 83.6 & 70.0 & 47.1 & 44.1 & \\
                  & 2  & 55.7 & 73.2 & 42.4 & 76.4 & 57.0 & 19.9 & 86.7 & 84.2 & 77.8 & 60.4 & 48.4 & \\
CoOp      & 4  & 57.9 & 75.4 & 45.7 & 77.0 & 61.4 & 22.7 & 87.2 & 85.5 & 84.8 & 69.4 & 53.4 & 65.5 \\
                  & 8  & 60.5 & 76.7 & 49.7 & 77.8 & 65.5 & 26.3 & 87.8 & 87.4 & 89.9 & 76.5 & 58.7 & \\
                  & 16 & 62.3 & 78.4 & 53.3 & 79.3 & 70.5 & 30.1 & 88.4 & 89.6 & 93.4 & 81.4 & 65.0 & \\
          \midrule
                  & 1  & 61.8 & 74.6 & 47.8 & 80.8 & 60.1 & 22.2 & 88.2 & 86.7 & 77.5 & 58.5 & 50.9 & \\
                  & 2  & 62.3 & 76.4 & 49.4 & 80.6 & 63.7 & 24.8 & 88.4 & 87.1 & 85.2 & 69.0 & 56.2 & \\
ProDA~\cite{Lu2022PromptDL}       & 4  & 63.6 & 78.3 & 51.7 & 80.8 & 67.9 & 27.5 & 89.0 & 88.7 & 90.6 & 75.3 & 60.0 & 70.3 \\
                  & 8  & 64.7 & 79.6 & 54.3 & 81.7 & 72.1 & 31.5 & 89.4 & 89.8 & 93.6 & 80.1 & 65.0 & \\
                  & 16 & 65.3 & 80.9 & 57.0 & 82.4 & 75.5 & 36.6 & 90.0 & 91.3 & 95.5 & 84.3 & 70.1 & \\
          \midrule
          & 1  &  &  &  &  &  &  &  &  &  &  &  &  \\
                  & 2  &  &  &  &  &  &  &  &  &  &  &  &  \\
POMP       & 4  & $63.7_\impro{0.1}$ & $79.8_\impro{1.5}$ & $52.1_\impro{0.4}$ & $79.5_\degra{1.3}$ & $68.0_\impro{0.1}$ & $27.3_\degra{0.2}$ & $89.2_\impro{0.2}$ & $91.6_\impro{2.9}$ & $93.1_\impro{2.5}$ & $82.7_\impro{7.4}$ & $60.9_\impro{0.9}$ & $71.6_\impro{1.3}$ \\
(Ours)            & 8  &  &  &  &  &  &  &  &  &  &  &  &  \\
                  & 16 &  &  &  &  &  &  &  &  &  &  &  &  \\
          \bottomrule
       
    \end{tabular}
    \end{adjustbox}
    \caption{Detailed performance (\%) of various methods on the $11$ downstream datasets. ``\# Shot'' denotes the number of training samples per class.}
    \label{tab:ft-ic}
\end{table*}



% \begin{table*}[htbp]
%     \centering
%     \footnotesize
%     \begin{tabular}{cccccccccccccc}
%         Method & \# Shot & 
%         \rotatebox{90}{ImageNet} & 
%         \rotatebox{90}{CIFAR-10} & 
%         \rotatebox{90}{CIFAR-100} & 
%          \rotatebox{90}{STL-10} &
%          \rotatebox{90}{Food-101} &
%          \rotatebox{90}{Stanford Cars} &
%          \rotatebox{90}{FGVC Aircraft} &
%          \rotatebox{90}{Oxford Pets} &
%          \rotatebox{90}{Caltech-101} &
%          \rotatebox{90}{Oxford Flowers} &
%          \rotatebox{90}{EuroSAT} &
%          \rotatebox{90}{DTD} \\
%          \toprule
%       Zero-Shot CLIP & 0  & 59.8 & 71.6 & 40.6 & 94.4 & 80.6 & 54.3 & 17.0 & 85.5 & 84.5 & 65.5 & 41.8 & 41.2 \\
%       \midrule
%                   & 1  & 22.1 & 44.3 & 18.2 & 80.6 & 31.4 & 24.3 & 13.0 & 30.2 & 56.7 & 56.1 & 46.8 & 29.8 \\
%                   & 2  & 31.9 & 53.5 & 26.6 & 86.9 & 45.1 & 36.8 & 17.9 & 40.5 & 68.7 & 74.9 & 55.5 & 41.4 \\
% Linear Probe CLIP  & 4  & 41.4 & 62.2 & 35.6 & 92.2 & 56.8 & 49.5 & 23.9 & 56.4 & 79.0 & 86.3 & 65.7 & 51.9 \\
%                   & 8  & 49.4 & 70.1 & 43.6 & 94.3 & 67.1 & 61.2 & 29.4 & 67.5 & 84.3 & 91.5 & 75.1 & 59.0 \\
%                   & 16 & 55.9 & 73.8 & 50.5 & 95.0 & 73.7 & 70.0 & 36.0 & 75.1 & 87.3 & 95.6 & 80.7 & 64.3 \\
%           \midrule
%                   & 1  & 53.4 & 71.8 & 41.3 & 94.1 & 77.5 & 54.0 & 17.7 & 86.5 & 83.6 & 70.0 & 47.1 & 44.1 \\
%                   & 2  & 55.7 & 73.2 & 42.4 & 94.3 & 76.4 & 57.0 & 19.9 & 86.7 & 84.2 & 77.8 & 60.4 & 48.4 \\
% CoOp      & 4  & 57.9 & 75.4 & 45.7 & 94.9 & 77.0 & 61.4 & 22.7 & 87.2 & 85.5 & 84.8 & 69.4 & 53.4 \\
%                   & 8  & 60.5 & 76.7 & 49.7 & 95.3 & 77.8 & 65.5 & 26.3 & 87.8 & 87.4 & 89.9 & 76.5 & 58.7 \\
%                   & 16 & 62.3 & 78.4 & 53.3 & 95.6 & 79.3 & 70.5 & 30.1 & 88.4 & 89.6 & 93.4 & 81.4 & 65.0 \\
%           \midrule
%                   & 1  & 61.8 & 74.6 & 47.8 & 95.1 & 80.8 & 60.1 & 22.2 & 88.2 & 86.7 & 77.5 & 58.5 & 50.9 \\
%                   & 2  & 62.3 & 76.4 & 49.4 & 95.3 & 80.6 & 63.7 & 24.8 & 88.4 & 87.1 & 85.2 & 69.0 & 56.2 \\
% ProDA       & 4  & 63.6 & 78.3 & 51.7 & 95.7 & 80.8 & 67.9 & 27.5 & 89.0 & 88.7 & 90.6 & 75.3 & 60.0 \\
%                   & 8  & 64.7 & 79.6 & 54.3 & 96.1 & 81.7 & 72.1 & 31.5 & 89.4 & 89.8 & 93.6 & 80.1 & 65.0 \\
%                   & 16 & 65.3 & 80.9 & 57.0 & 96.3 & 82.4 & 75.5 & 36.6 & 90.0 & 91.3 & 95.5 & 84.3 & 70.1 \\
%           \midrule
%           & 1  &  &  &  &  &  &  &  &  &  &  &  &  \\
%                   & 2  &  &  &  &  &  &  &  &  &  &  &  &  \\
% POMP (Ours)       & 4  &  &  &  &  &  &  &  &  &  &  &  &  \\
%                   & 8  &  &  &  &  &  &  &  &  &  &  &  &  \\
%                   & 16 &  &  &  &  &  &  &  &  &  &  &  &  \\
%           \bottomrule
       
%     \end{tabular}
%     \caption{Detailed performance (\%) of various methods on the $12$ downstream datasets. ``\# Shot'' denotes the number of training samples per class.}
%     \label{tab:res}
% \end{table*}


==> tables/ic_cross_dataset.tex <==
\begin{table*}[h!]
    % \tabstyle{5pt}
\caption{Comparison of CART with existing approaches on cross-dataset evaluation. Overall, CART achieves competitive performance providing highest average accuracy, indicating better generalization.}
\label{tab:ic-cross-dataset}
\vskip 0.15in
\begin{adjustbox}{max width=\textwidth}

\begin{tabular}{l c ccccccccccc}
\toprule
& \textbf{Source} & \multicolumn{11}{c}{\textbf{Target}} \\ \cmidrule(lr){2-2} \cmidrule(lr){3-13}
& \rotbox{ImageNet} & \rotbox{Caltech101} & \rotbox{OxfordPets} & \rotbox{StanfordCars} & \rotbox{Flowers102} & \rotbox{Food101} & \rotbox{Aircraft} & \rotbox{SUN397} & \rotbox{DTD} & \rotbox{EuroSAT} & \rotbox{UCF101} & \rotbox{\emph{Average}} \\
\midrule
CoOp~\cite{Zhou2022LearningTP} & \textbf{71.51} & 93.70 & 89.14 & 64.51 & 68.71 & 85.30 & 18.47 & 64.15 & 41.92 & {46.39} & 66.55 & 63.88 \\
CoCoOp~\cite{Zhou2022ConditionalPL} & 71.02 & 94.43 & 90.14 & 65.32 & 71.88 & 86.06 & 22.94 & 67.36 & 45.73 & 45.37 & 68.21 & 65.74 \\
% CPT & 71.90 & 94.20 & 90.30 & 64.50 & 70.90 & 86.30 & 21.70 & 66.80 & 45.30 & 47.70 & 69.30 & 65.70 \\
LASP~\cite{Bulat2022LanguageAwareSP} & 71.10 & 94.50 & 89.36 & 64.83 & 70.53 & 86.30 & 23.03 & 67.00 & 45.54 & 48.33 & 68.24 & 65.77 \\
VPT~\cite{Derakhshani2022VariationalPT} & 70.70 & 93.67 & \textbf{90.63} & 65.00 & 70.90 & 86.30 & 24.93 & 67.47 & 46.10 & 45.87 & 68.67 & 65.95 \\
MaPLe~\cite{Khattak2022MaPLeMP} & 70.72 & 93.53 & 90.49 & 65.57 & 72.23 & 86.20 & 24.74 & 67.01 & \textbf{46.49} & 48.06 & \textbf{68.69} & 66.30 \\
\midrule
\rowcolor{tabhighlight} POMP (Ours) & 70.20 & \textbf{95.01} & 89.51 & \textbf{66.77} & \textbf{72.43} & \textbf{86.30} & \textbf{25.56} & \textbf{67.71} & 46.22 & \textbf{52.05} & 68.54 & \textbf{67.01} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\vskip -0.1in
\end{table*}

==> tables/ic_cross_domain.tex <==
\begin{table*}[h!]
\caption{ Comparison of CART with existing approaches in domain generalization setting. CART shows highest performance on all target datasets.
}
\label{tab:ic-cross-domain}
\vskip 0.15in
\centering
\begin{adjustbox}{max width=.8\textwidth}
\begin{tabular}{l cccccc}
\toprule
& \textbf{Source} & \multicolumn{5}{c}{\textbf{Target}} \\ \cmidrule(lr){2-2} \cmidrule(lr){3-7}
 & ImageNet & ImageNetV2 & ImageNet-Sketch & ImageNet-A & ImageNet-R & Average \\
\midrule
CLIP~\cite{Radford2021LearningTV} &  66.73 & 60.83 & {46.15} & 47.77 & {73.96} & 57.18 \\
CoOp~\cite{Zhou2022LearningTP} &  \textbf{71.51} & 64.20 & 47.99  & 49.71  & 75.21 & 59.28 \\
CoCoOp~\cite{Zhou2022ConditionalPL} & 71.02 & 64.07 & 48.75 & 50.63 & 76.18 & 59.91  \\
MaPLe~\cite{Khattak2022MaPLeMP} & 70.72 & 64.07 & 49.15 & 50.90  & 76.98 & 60.28 \\
% CPT &  71.90 & 64.60 & 49.20 & 51.10 & 76.80 & 60.43 \\
LASP~\cite{Bulat2022LanguageAwareSP} & 71.10 & 63.77 & 49.01 & 50.70 & 77.07 & 60.14 \\
VPT~\cite{Derakhshani2022VariationalPT} &  70.70 & \textbf{64.23} & 49.20 & 51.33 & 77.00 & 60.44 \\
\midrule
\rowcolor{tabhighlight} POMP (Ours) & 70.20 & 63.80 & \textbf{49.79} & \textbf{51.56}  & \textbf{77.85} & \textbf{60.75} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\vskip -0.1in
\end{table*}

==> tables/lvis.tex <==
\begin{table*}[t]
\small
\centering
\begin{tabular}{l|c|cccc|cccc}
\toprule
\multirow{2}{*}{Method}&\multirow{2}{*}{Epoch}&\multicolumn{4}{c|}{Detection}&\multicolumn{4}{c}{Instance segmentation}\\
&&AP$_{r}$&\textcolor{grey}{AP$_{c}$}&\textcolor{grey}{AP$_{f}$}&\textcolor{grey}{AP}&AP$_{r}$&\textcolor{grey}{AP$_{c}$}&\textcolor{grey}{AP$_{f}$}&\textcolor{grey}{AP}\\
\midrule
Supervised (base)& 20 &0.0&\textcolor{grey}{26.1}&\textcolor{grey}{34.0}&\textcolor{grey}{24.7}&0.0&\textcolor{grey}{24.7}&\textcolor{grey}{29.8}&\textcolor{grey}{22.4}\\
Supervised (base+novel)& 20 &15.5&\textcolor{grey}{25.5}&\textcolor{grey}{33.6}&\textcolor{grey}{27.0}&16.4&\textcolor{grey}{24.6}&\textcolor{grey}{30.6}&\textcolor{grey}{25.5}\\
\midrule
ViLD (base)\cite{gu2021zero} &460 &16.7&\textcolor{grey}{26.5}&\textcolor{grey}{34.2}&\textcolor{grey}{27.8}&16.6&\textcolor{grey}{24.6}&\textcolor{grey}{30.3}&\textcolor{grey}{25.5}\\
ViLD* (base)~\cite{gu2021zero}  & 20 &17.4&\textcolor{grey}{27.5}&\textcolor{grey}{31.9}&\textcolor{grey}{27.5}&16.8&\textcolor{grey}{25.6}&\textcolor{grey}{28.5}&\textcolor{grey}{25.2}\\
DetPro (base)~\cite{Du2022LearningTP} & 20 & \textbf{20.8} &\textcolor{grey}{27.8}&\textcolor{grey}{32.4}&\textcolor{grey}{28.4}& \textbf{19.8} &\textcolor{grey}{25.6}&\textcolor{grey}{28.9}&\textcolor{grey}{25.9}\\
%ViLD text+prompt 1x(ours)&15.8&26.2&32.9&27.0&14.9&24.2&28.9&24.4\\
\midrule
Detic~\cite{Zhou2022DetectingTC} & ? & 26.7 &\textcolor{grey}{36.4}&\textcolor{grey}{40.3}&\textcolor{grey}{36.3}& 24.9 &\textcolor{grey}{32.5}&\textcolor{grey}{35.6}&\textcolor{grey}{32.4}\\
% POMP (Ours) & ? & \textbf{26.8} &\textcolor{grey}{36.3}&\textcolor{grey}{40.3}&\textcolor{grey}{36.2}& 24.8 &\textcolor{grey}{32.8}&\textcolor{grey}{35.5}&\textcolor{grey}{32.5}\\
POMP (Ours) & ? & \textbf{26.8} &\textcolor{grey}{36.4}&\textcolor{grey}{40.4}&\textcolor{grey}{36.2}& \textbf{25.2} &\textcolor{grey}{33.0}&\textcolor{grey}{35.6}&\textcolor{grey}{32.7}\\
\midrule
Detic~\cite{Zhou2022DetectingTC} (Box-Supervised) & ? & 17.6 &\textcolor{grey}{34.4}&\textcolor{grey}{40.3}&\textcolor{grey}{33.8}& 16.4 &\textcolor{grey}{31.0}&\textcolor{grey}{35.4}&\textcolor{grey}{30.2}\\
POMP (Ours) & ? & \textbf{20.3} &\textcolor{grey}{33.7}&\textcolor{grey}{39.9}&\textcolor{grey}{33.8}& \textbf{19.2} &\textcolor{grey}{30.3}&\textcolor{grey}{35.2}&\textcolor{grey}{30.3}\\
\bottomrule
\end{tabular}
% \vspace{-2mm}
\caption{Comparison with ViLD on LVIS v1 dataset. * denotes our re-implementation version, see Section~\ref{sec:details} for the details. The frequent and common  classes are used as the base classes, while the rare classes are held out as the novel classes. $\text{AP}_r$ is the main evaluation metric for open-world object detection.}
% \vspace{-2mm}
\label{tab:openvocab}
\end{table*}

==> tables/ss_ov_cocostuff.tex <==
\begin{table}[]
    \small
    \centering
    \begin{tabular}{l|c|c|c|c}
    \toprule
    \multirow{2}{*}{Method}&\multirow{2}{*}{hIoU} & \multirow{2}{*}{pAcc}&\multicolumn{2}{c}{mIoU}\\
      \cline{4-5}
     &&&seen&unseen\\
    \midrule
      SPNet~\cite{Xian2019SemanticPN}&16.8&-&20.5&14.3\\
      ZS3~\cite{Bucher2019ZeroShotSS}&15.0&-&34.7&9.5\\
      CaGNet~\cite{Gu2020ContextawareFG}&18.2&-&35.5&12.2\\
      ZSSeg~\cite{Xu2021ASB}&37.8&\textbf{60.3}&39.3&36.3\\
      POMP (Ours) & \textbf{39.1} & 59.0 & \textbf{39.9} & \textbf{38.2}\\
    \bottomrule
    \end{tabular}
    \caption{Comparison with state-of-the-art methods on the validation set of COCO Stuff dataset.}
    \label{tab:coco_stuff_res}
\end{table}  

==> tables/ss_ov_pascalvoc.tex <==
\begin{table}[]
    \small
    \centering
    \begin{tabular}{l|c|c|c|c}
    \toprule
    \multirow{2}{*}{Method}&\multirow{2}{*}{hIoU} & \multirow{2}{*}{pAcc}&\multicolumn{2}{c}{mIoU}\\
      \cline{4-5}
     &&&seen&unseen\\
    \midrule
    SPNet~\cite{Xian2019SemanticPN}&21.8         &-        & 73.3                                   & 15.0                 \\
    ZS3~\cite{Bucher2019ZeroShotSS}&28.7             &-    & 77.3                                    & 17.7                 \\
    CaGNet~\cite{Gu2020ContextawareFG}&39.7             &-    & 78.4                                              & 25.6                 \\
    
    ZSSeg~\cite{Xu2021ASB}&77.5       &90.0         & 83.5 & 72.5                \\
    ZSSeg (re)~\cite{Xu2021ASB}&70.4       &93.0         & 93.3 & 56.6                \\
    POMP (Ours) & \textbf{84.4} & \textbf{95.6} & \textbf{93.6} & \textbf{76.8}\\
    \bottomrule
    \end{tabular}
    \caption{Comparison with state-of-the-art methods on the validation set of Pascal VOC dataset.}
    \label{tab:pascal_voc_res}
\end{table} 

==> tables/ss_ov_var_prompt.tex <==
\begin{table}[]
\caption{Comparison with state-of-the-art methods on the validation set of COCO Stuff dataset and Pascal VOC dataset.}%, respectively. POMP and ZSSeg share the same mask proposal network and training strategy.}
\label{tab:ss-ov}
\vskip 0.15in
\small
\centering
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{l|ccc|ccc}
\toprule
\multirow{3}{*}{Method} & \multicolumn{3}{c|}{Open-Vocab COCO Stuff}                                      & \multicolumn{3}{c}{Open-Vocab Pascal VOC}                                       \\ \cline{2-7} %\cmidrule(lr){2-4} \cmidrule(lr){5-7} 
                        & \multicolumn{1}{c|}{\multirow{2}{*}{hIoU}} & \multicolumn{2}{c|}{mIoU}          & \multicolumn{1}{c|}{\multirow{2}{*}{hIoU}} & \multicolumn{2}{c}{mIoU}           \\ \cline{3-4} \cline{6-7} % \cmidrule(lr){3-4} \cmidrule(lr){6-7} 
                        & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c|}{seen} & unseen & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c|}{seen} & unseen \\ \midrule
ZSSeg (single prompt)    & \multicolumn{1}{c|}{33.6}                  & \multicolumn{1}{c|}{40.1} &  28.8  & \multicolumn{1}{c|}{-}                  & \multicolumn{1}{c|}{-} & -   \\
POMP (Ours)             & \multicolumn{1}{c|}{\textbf{36.8}}                  & \multicolumn{1}{c|}{\textbf{40.1}} & \textbf{34.1}   & \multicolumn{1}{c|}{\textbf{-}}                  & \multicolumn{1}{c|}{\textbf{-}} & \textbf{-}   \\ \bottomrule
\end{tabular}
\end{adjustbox}
\vskip -0.1in
\end{table}  

==> tables/vqa.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\begin{tabular}{@{}lcccc@{}}
\toprule
n-shot Acc.      & n=1   & n=4   & n=16  & n=32  \\ \midrule
Fronzen\_blind   & 33.50 & 33.30 & -     & -     \\
Frozen           & 35.70 & 38.20 & -     & -     \\
TAP-C (ViT-B/16) & 43.27 & 44.98 & 47.42 & 49.19 \\
TAP-C (Res50x16) & 43.24 & 45.87 & 48.89 & 50.18 \\
PICa-Base        &       &       & 54.3  &       \\
PICa-Full        &       &       & 56.1  &       \\ \midrule
EPT (Ours)       &       &       &       &       \\ \bottomrule
\end{tabular}
\caption{few-shot VQAv2}
\end{table}
